Scalable Lattice Influence Maximization

Influence maximization is the task of finding k seed nodes in a social network such that the expected number of activated nodes in the network (under certain influence propagation model), referred to as the influence spread, is maximized. Lattice influence maximization (LIM) generalizes influence maximization such that, instead of selecting k seed nodes, one selects a vector x = (x_1, ..., x_d) from a discrete space X called a lattice, where x_j corresponds to the j-th marketing strategy and x represents a marketing strategy mix. Each strategy mix x has probability h_u(x) to activate a node u as a seed.LIM is the task of finding a strategy mix under the constraint x_1+...+x_d <= k such that its influence spread is maximized. We adapt the reverse influence sampling (RIS) approach and design scalable algorithms for LIM. We first design the IMM-PRR algorithm based on partial reverse-reachable sets as a general solution for LIM, and improve IMM-PRR for a large family of models where each strategy independently activates seed nodes. We then propose an alternative algorithm IMM-VSN based on virtual strategy nodes, for the family of models with independent strategy activations. We prove that both IMM-PRR and IMM-VSN guarantees 1-e-\epsilon approximation for small \epsilon> 0. Empirically, through extensive tests we demonstrate that IMM-VSN runs faster than IMM-PRR and much faster than other baseline algorithms while providing the same level of influence spread. We conclude that IMM-VSN is the best one for models with independent strategy activations, while IMM-PRR works for general modes without this assumption. Finally, we extend LIM to the partitioned budget case where strategies are partitioned into groups, each of which has a separate budget, and show that a minor variation of our algorithms would achieve 1/2 -\epsilon approximation ratio with the same time complexity.

==> alternative.tex <==
\section{Alternative RR Set Construction via Pseudo Nodes}

When applying the reverse influence sampling (RIS) approach to the LIM problem, our
	key connection is the Eq.~\eqref{eq:RRSetGMS} in Lemma~\ref{lem:RRSetGMS}:
	it connects the influence spread $g(\vx)$ with the expectation of
	a fraction $1 - \prod_{v\in R}(1 - h_v(\vx))$, where the expectation is taken over
	the random RR set $R$.
The fractional expectation makes the design of an efficient hill-climbing algorithm on
	RR sets more complicated (Section~\ref{sec:application}) than the
	original {\IMM} algorithm, which is based on equation 
	$\sigma(S) = n \cdot \E_R[\I\{S\cap R \neq \emptyset\}]$, where the expectation is on
	a simple indicator random variable $\I\{S\cap R \neq \emptyset\}$.
	
One may try an alternative approach, which converts the LIM propagation model into 
	an equivalent IC model by adding {\em pseudo nodes} representing strategies
	and {\em pseudo edges} representing relationship from strategies to nodes
	into the social graph $G$.
The hope is that we could then apply the original {\IMM} algorithm on the new graph to
	obtain the greedy strategy mix directly.
However, this approach has its own issues, as we discuss now in this section.

In the following, we assume that Eq.~\eqref{eq:hv} holds, that is, every strategy $j$
	has independent influence on every node $v$, since this is close to the spirit
	of the IC model.

\subsection{Alternative 1}

For every strategy $j$, we construct pseudo nodes $u_{j,1}, u_{j,2}, \ldots, u_{j,k\delta^{-1}}$, 
	where $u_{j,i}$ corresponds to the quantity of strategy $j$, $x_j = i\delta$.
For every pseudo node $u_{j,i}$ and every node $v$ in the original graph, 
	we construct a direct pseudo edge from $u_{j,i}$ to $v$, with influence probability
\begin{equation} \label{eq:fromqtoedgeprob}
p(u_{j,i},v) = \frac{q_{v,j}(i\delta) - q_{v,j}((i-1)\delta)}{1 - q_{v,j}((i-1)\delta)}, j\ge 1.
\end{equation}

With the above construction, when we select $x_j = i\delta$ for strategy $j$, it corresponds to
	selecting nodes $u_{j,1}, \ldots, u_{j,i}$ as seed nodes, because for every node $v$
	in graph $G$, the probability of
	these seed nodes activating $v$ is exactly $q_{v,j}(x_j) = q_{v,j}(i\delta)$.
This can be proven by an induction on $i$.
When $i=1$, the probability of activating $v$ is simply 
\begin{equation*}
p(u_{j,1},v) = \frac{q_{v,j}(\delta) - q_{v,j}(0)}{1 - q_{v,j}(0)} = q_{v,j}(\delta).
\end{equation*}
For general $i > 1$, using the induction hypothesis, we derive that the probability of
	seed nodes $u_{j,1}, \ldots, u_{j,i}$ activating $v$ as:
\begin{align*}
& 1- \prod_{t=1}^i (1-p(u_{j,t},v)) \\
& = 1 - (1-q_{v,j}((i-1)\delta))\cdot (1-p(u_{j,i},v)) \\
& = 1- (1-q_{v,j}((i-1)\delta)) \left( 1 - 
	\frac{q_{v,j}(i\delta) - q_{v,j}((i-1)\delta)}{1 - q_{v,j}((t-1)\delta)} \right) \\
& = q_{v,j}(i\delta).
\end{align*}
Thus, strategy $x_j = i\delta$ is indeed equivalent of selecting seed nodes 
	$u_{j,1}, \ldots, u_{j,i}$.
In general, for any strategy mix $\vx = (x_1, \ldots, x_d)$, it corresponds to 
	seed nodes $\{u_{j,i} \mid j= 1, \ldots, d, 1\le i \le x_j \delta^{-1}\}$.
Let $G_A$ be the augmented graph constructed above.
In other words, the propagation model in LIM from the strategy mix $\vx$
	is equivalently represented as an IC model propagation in the graph $G_A$ from
	seed nodes $\{u_{j,i} \mid j= 1, \ldots, d, 1\le i \le x_j \delta^{-1}\}$.
Therefore, it looks like that we could solve the LIM problem by 
	solving the classical influence maximization problem in the IC model on graph $G_A$, as
	long as we restrict that only the pseudo nodes could be selected as seeds.
	
\wei{The following are more like ideas. It will not be the final presentation in the paper.}

However, the extra restriction that for each strategy $j$, the seed set for $j$ must be
	a prefix of nodes $u_{j,1}, \ldots, u_{j, k\delta^{-1}}$ may cause problems.
When we apply the IC model influence maximization on graph $G_A$, we may not obtain
	a prefix seed set for $j$.
Suppose $S_j \subseteq \{ u_{j,1}, \ldots, u_{j, k\delta^{-1}}\}$ is the seed set selected
	for strategy $j$.
We cannot claim that replacing $S_j$ to the prefix $u_{j,1}, \ldots, u_{j,|S_j|}$ would give
	a better result.
Then we cannot simply map $S_j$ with $x_j = |S_j|\cdot \delta$ to claim that the obtained
	strategy mix $\vx = (x_1, \ldots, x_d)$ is an approximate solution to the LIM problem.
The issue is that, due to the IC model, there is a denominator in Eq.~\eqref{eq:fromqtoedgeprob},
	and thus even if $q_{v,j}$ is concave, we can only relax the numerator of
	Eq.~\eqref{eq:fromqtoedgeprob} to a smaller index $i$, but not the whole fraction.

The solution seems to be getting rid of the denominator in Eq.~\eqref{eq:fromqtoedgeprob} , which
	means getting rid of the IC model for the part from pseudo nodes to actual nodes.
In fact, the linear threshold (LT) model can do the job here.

We construct the graph $G_A$ as before, but for each edge $(u_{j,i},v)$, instead of assigning
	an influence probability as for the IC model, we assign the following influence weight
	as for the LT model.
\begin{equation} \label{eq:fromqtoedgeweight}
w(u_{j,i},v) = q_{v,j}(i\delta) - q_{v,j}((i-1)\delta), j\ge 1.
\end{equation}
Recall that for the LT model, the node $v$ is activated with probability 
	equal the sum of weights of incoming edges from activated in-neighbors.
Therefore, when $u_{j,1}, \ldots, u_{j,i}$ are selected as seed nodes, the probability
	that $v$ is activated is exactly 
	$\sum_{t=1}^i w(u_{j,t},v) = q_{v,j}(i\delta)$.
Moreover, when $q_{v,j}$ is monotone increasing and concave, we have
	$w(u_{j,1},v) \ge w(u_{j,2},v) \ge \cdots \ge w(u_{j,k\delta^{-1}},v)$.
Hence, for any subset of $\{  u_{j,1}, \ldots, u_{j, k\delta^{-1}}\}$ of size $i$, 
	the set that activates $v$ with the largest probability is exactly
	the prefix set $\{u_{j,1}, \ldots, u_{j,i} \}$.
This means that for any seed set for $G_A$, we can always find a corresponding
	strategy mix vector $\vx$ that has influence spread no worst than the seed set.
This means that any approximate solution in the $G_A$ model can be translated to an approximate
	solution for LIM.
Therefore, the above is a correct conversion from LIM to a classical influence model.

Notice that the model in $G_A$ is not IC or LT model, but a mixed IC and LT model.
But since both IC and LT belongs to the triggering model, it is still a valid triggering model.
Since any triggering model allows the use of the {\IMM} algorithm, we can apply {\IMM} to 
	the above converted model.
In particular, for the LT part of the above model, when we reverse simulate from $v$ 
	to pseudo nodes for strategy $j$, the LT model implies that we only select
	one edge $(u_{j,i},v)$ with probability proportional to weight $w(u_{j,i},v)$.
However, between two different strategies $j$ and $j'$, or between strategy $j$ and
	a regular in-neighbor $w$ of $v$, their attempt of activating $v$ are still independent,
	and thus the reverse simulation for them are generated independently.
This is really a mixed IC and LT model.

Now we need to check the time complexity of this approach. 
For $G_A$, we add  $d k\delta^{-1}$ nodes and $ k\delta^{-1} \sum_{v\in V} |S_v|$ edges.
Thus, the expected running time for running {\IMM} on $G_A$ is 
	$O((k+\ell)(m +  k\delta^{-1}\sum_{v\in V} |S_v|) \log (n + d k\delta^{-1}) /\varepsilon^2)$.
When we consider that the influence spread range is still upper bounded by $n$, 
	the possible seed set choices is upper bounded by $d^{k\delta^{-1}}$ (so we can
	replace  $\ln \binom{n}{k}$ with $k \delta^{-1} \ln d$), I believe we can
	fine tune the expected running time to
	$O((k\log n +\ell \log n + k \delta^{-1} \log d)(m + k\delta^{-1}\sum_{v\in V} |S_v|) /\varepsilon^2)$.
Comparing with 
	$O(k\delta^{-1}T_q(\max_{v\in V}|S_v|)(k\delta^{-1} \log d+\ell\log n)(n + m)/  \varepsilon^2)$
	in Theorem~\ref{thm:IMMGMS}, 
	first, $T_q$ for computing $q_{v,j}$ once can be removed on both cases by preprocessing,
	so it does not make much difference.
The term $(k\log n +\ell \log n + k \delta^{-1} \log d)$ is more or less comparable with
	$(k\delta^{-1} \log d+\ell\log n)$
\wei{perhaps we should add $k \log n$ to the {\IMMGMS} algorithm too?}.
Thus, the main differentiating factors are
	$(m + k\delta^{-1}\sum_{v\in V} |S_v|)$ for the new alternative
	versus $k\delta^{-1}\max_{v\in V}|S_v|(m+n)$ for {\IMMGMS}.
Since $	m + k\delta^{-1}\sum_{v\in V} |S_v| \le m + k\delta^{-1} n \max_{v\in V} |S_v|
	\le k\delta^{-1}\max_{v\in V}|S_v| (m+n)$, it looks like the alternative
	approach is competitive or may be slightly better than the {\IMMGMS} algorithm.
	
One possible way of improving the alternative approach, is when reverse simulating
	the LT part for strategy $j$, we assume it would take $O(k\delta^{-1})$ time to generate
	the reverse edge, but perhaps for the LT model with the $q_{v,j}$ function, we can
	do it by binary search, in $O(\log (k\delta^{-1}))$ time.
%But the factor of $d$ seems to be still there.

\wei{The above is my new idea so far. 
I think it has the same spirit as what the reviewer in KDD18 suggested, but that reviewer
	only mentioned using IC model, while I think IC model itself won't work, and we need the
	above mixed IC and LT model.
This sounds a new technical contribution now, and it is indeed worth to do some tests on that.
It is possible that the two approach will win in different cases.

Also, I can't recall what is the other alternative. 

In any case, this part seems to be something new, and we cannot include it here I guess.}

%\wei{There are several issues here.
%(a) The seed set has to be a prefix. Can we argue that if it is not a prefix for a certain
%strategy, then it is always better to move the seeds ahead to form a prefix? I don't think
%this holds. Note that both the reviewer comment and the previous WWW18 submission 
%	construct edge probabilities similar to Eq.~\ref{eq:fromqtoedgeprob}, but ignoring
%	the denominator. When ignoring the denominator, we simply assuming the combined
%	effect of a seed set is a summation of edge probabilities, which does not hold for
%	the IC model, but works for the LT model. Without the denominator, it seems we can argue
%	that the prefix is always better, by the concaveness of function $q_{v,j}$.
%But with the denominator, I don't think it holds.
%Does this mean that we have to use the LT threshold model from pseudo nodes to actual nodes?
%Perhaps it is ok if we do so.
%
%(b) When we construct RR sets, is there a submodularity violation issue, as we see in 
%	the WWW18 submission? I feel that if we restrict that the seed set has to be a prefix, then
%	when generating RR set, we may not get a prefix, and there is an issue. But if
%	we do not restrict seed set to be a prefix, then it is ok. That means, if we use the
%	LT model from pseudo nodes to actual nodes, then perhaps it is ok. But in this case,
%	when covering seed set to strategy, for strategy $j$, we should only count the number of 
%	pseudo nodes selected for strategy $j$, and multiply it with $\delta$ to get the
%	$x_j$.
%	
%(c) In terms of the complexity, we add $d k\delta^{-1}$ nodes and $n d k\delta^{-1}$
%	edges. Is this better or worse comparing to our current solution?
%}

\subsection{Alternative 2}




